BARD: Bridging AutoRegressive and Diffusion Vision-Language Models Via Highly Efficient Progressive Block Merging and Stage-Wise Distillation

Autoregressive vision-language models (VLMs) deliver strong multimodal capability, but their token-by-token decoding imposes a fundamental inference bottleneck. Diffusion VLMs offer a more parallel decoding paradigm, yet directly converting a pretrained autoregressive VLM into a large-block diffusion VLM (dVLM) often leads to substantial quality degradation. In this work, we present BARD, a simple and effective bridging framework that converts a pretrained autoregressive VLM into a same-architecture, decoding-efficient dVLM. Our approach combines progressive supervised block merging, which gradually enlarges the decoding block size, with stage-wise intra-dVLM distillation from a fixed small-block diffusion anchor to recover performance lost at larger blocks. We further incorporate a mixed noise scheduler to improve robustness and token revision during denoising, and memory-friendly training to enable efficient training on long multimodal sequences. A key empirical finding is that direct autoregressive-to-diffusion distillation is poorly aligned and can even hurt performance, whereas distillation within the diffusion regime is consistently effective. Experimental results show that, with $\leq$ 4.4M data, BARD-VL transfers strong multimodal capability from Qwen3-VL to a large-block dVLM. Remarkably, BARD-VL establishes a new SOTA among comparable-scale open dVLMs on our evaluation suite at both 4B and 8B scales. At the same time, BARD-VL achieves up to 3$\times$ decoding throughput speedup compared to the source model. Code is available at https://github.com/fudan-generative-vision/Bard-VL.

==> preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> section/dstar.tex <==
 \begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/architecture.pdf}
    \caption{Overall architecture and training framework of the BARD Vision-Language Model (BARD-VL).
    (a) Pipeline: Illustrates the packed vectorized training layout $[Q, x_1, x_t]$ and highlights the paradigm shift by contrasting the vanilla dLLM target (struck-through Vanilla Objective) with the proposed Mixed Noise Objective ($\mathcal{L}_{mixed}$). This objective is optimized over the union of masked and uniformly corrupted positions $\mathcal{S}_t = \mathcal{M}_t \cup \mathcal{U}_t$.
    (b) Attention Mask: A comparision between the vanilla mask ($e.g., \cite{arriola2025block, cheng2510sdar}$) and ours.
    While vanilla block-wise attention mask used allow perturbed blocks $\in [Q, \; x_t]$ to attend to all preceding clean blocks $\in [Q, \; x_1]$, the attention mask of BARD is specifically optimized for the packed vectorized layout $[Q,\; x_1,\; x_t]$.
    It ensures that the $i$-th token block in the noisy response $x_t^{i}$ attends only to the shared context $Q$, a causal prefix of the clean response $\{x_1^0, \dots, x_1^{i-1}\}$, and noisy tokens within the same generation block.
    (c): Mixed Noise: Visualizes the noise scheduling mechanism through the time-dependent coefficients $\kappa^1, \kappa^2, \mathrm{ and }~\kappa^3$.
    These coefficients govern the transition from the masked source to the clean target by blending absorbing-mask and uniform vocabulary noise.
    }
    \label{fig:architecture}
\end{figure*}

\section{BARD-VL}
\label{sec:model}

% \subsection{Packed Vectorized Training}
% \label{sec:packed-training}
The proposed bridging framework in Sec.~\ref{sec:method} is built upon a structural design tailored for multimodal inputs \(Q\), where visual tokens typically dominate the sequence length.
Vanilla discrete diffusion models ($e.g.,$ SDAR~\cite{cheng2025sdar}) often rely on a dual-sequence formulation that necessitates independently constructing the clean and perturbed sequences.
As illustrated by the vanilla block-wise attention mask in Figure~\ref{fig:architecture}~(b), this approach requires a redundant duplication of \(Q\) to form two separate input pairs: one for the clean target $([Q, \; x_1])$ and another for the perturbed state $([Q, x_t])$.
In multimodal settings, where high-resolution visual tokens from image or videos often dominate the sequence, this repetition severely restricts the effective context window and imposes a prohibitive memory bottleneck.
To resolve this, we propose the Packed Vectorized Layout (PVL) as a foundational sequence representation.
Instead of treating efficiency as a secondary optimization, PVL transforms it into an inherent structural property by unifying the shared context \(Q\) with the clean target $x_1$ and its noisy counterpart $x_t$ into a single sequence space:
\begin{equation}
\tilde{x} = [Q,\; x_1,\; x_t].
\label{eq:packed-sequence}
\end{equation}
By anchoring the noised response $x_t$ to a singular instance of \(Q\) and a causal prefix of the clean response $x_1$, BARD eliminates modal redundancy while enabling the model to process all diffusion blocks in a single, intergrated forward pass.
This unified representation naturally dictates the attention mechanism shown in Figure~\ref{fig:architecture}~(b).
While vanilla block-wise masks allow perturbed blocks to attend to duplicated prefixes, BARD's attention pattern is specifically architected to manage the intra-sequence dependencies within the $([Q, \; x_1])$ layout.
Tokens in the shared context \(Q\) and clean response $x_1$ retain their original causal dependencies to leverage the pretrained backbone's inherent reasoning capabilities.
For the noisy response $x_t$, the architecture enforces a selective visibility: it ensures that the $i$-th token block $x_t^i$ attends only to the shared context $Q$, a causal prefix of the clean response $\{x_1^0, \dots, x_1^{i-1}\}$, and noisy tokens within the same generation block. 
Crucially, the block-diagonal self-attention within $x_t$ acts as a structural constraint that ensures parallel independence, preventing information from future noisy blocks leaking into the current generating block.
By eliminating $Q$ redundancy, this consolidation expands the effective context window, thereby better fostering the emergence of sophisticated reasoning capabilities from the multimodal data.  

Beyond the sequence layout, and as an optional extension to the main bridging algorithm in Sec.~\ref{sec:method}, we further study a refinement module denoted as \modname. 
This module is not required by the main bridge and does not bring a large overall benchmark gain. 
Instead, its main benefit is qualitative: it enables the dVLM to revise low-confidence tokens during inference, rather than committing to the first materialized prediction.
Through this mechanism, and as highlighted by the contrast in Figure~\ref{fig:architecture}~(a), BARD evolves from the "reconstruction-only" focus of vanilla dLLMs (indicated by the struck-through Vanilla Objective) toward a Mixed Noise Objective ($\mathcal{L}_{mixed}$). 
The idea is simple. 
Standard absorbing-state diffusion only teaches the model to recover masked tokens.
In contrast, \modname\ additionally exposes the model to visible but corrupted tokens during training. Concretely, for each completion position \(i\), we sample the noised token from a mixed corruption process
\begin{equation}
q(x_t^i \mid x_1^i, t)
=
\alpha_t\,\delta_{\texttt{[MASK]}}(x_t^i)
+
\beta_t\,p_u(x_t^i)
+
(1-\alpha_t-\beta_t)\,\delta_{x_1^i}(x_t^i),
\label{eq:modname_corruption}
\end{equation}
where \(p_u\) is the uniform distribution over visible vocabulary tokens and \(\delta_a(\cdot)\) is a point mass at token \(a\). The first term is the standard mask corruption, while the second term replaces a token by a random visible token. As a result, the model is trained to handle both missing-token recovery and visible-token correction. Figure~\ref{fig:architecture}~(c) illustrates this mixed corruption process.
We optimize the same denoising objective as in standard diffusion training, but only on the corrupted positions:
\begin{equation}
\mathcal L_{\modname}(\theta)
=
-
\mathbb E_{(Q,x_1),\,x_t}
\left[
\frac{1}{\max(1,|\mathcal S_t|)}
\sum_{i\in\mathcal S_t}
\log p_\theta(x_1^i \mid x_t,Q)
\right],
\label{eq:modname_loss}
\end{equation}
where \(\mathcal S_t\) denotes the set of positions corrupted either by \texttt{[MASK]} replacement or by visible-token replacement.
At inference time, \modname\ uses a simple confidence-based refinement rule. Given the current prediction state \(x^{(s)}\), the model produces, for each completion position \(i\),
\begin{equation}
\hat{x}_i^{(s)}=\arg\max_{v\in\mathcal V} p_\theta(x_i=v\mid x^{(s)},Q),
\quad
c_i^{(s)}=\max_{v\in\mathcal V} p_\theta(x_i=v\mid x^{(s)},Q).
\label{eq:modname_confidence}
\end{equation}
Masked positions are first materialized when their confidence exceeds a threshold \(\eta\). For already visible positions, we allow revision if a later forward pass assigns a higher confidence than the previously accepted one. In this way, high-confidence tokens tend to stabilize early, while low-confidence tokens remain revisable and can be corrected when more context becomes available.
Therefore, \modname\ should be viewed as a refinement-oriented extension rather than a core part of the bridge. Its main effect is to improve the model's ability to revisit uncertain local decisions during decoding. In the experiments, we analyze this behavior through mixed-noise ablations and attention-map visualizations.

==> section/preliminary.tex <==
\section{Preliminaries}
\label{sec:prelim}

We consider the problem of converting a pretrained autoregressive vision-language model (VLM) into a same-architecture diffusion VLM (dVLM). Let \(Q\) denote the multimodal conditioning context, including the visual inputs and the textual prompt, and let \(x_1 \in \mathcal{V}^{L}\) denote the target completion sequence over vocabulary \(\mathcal{V}\). We use \(\mathcal{C}=\{1,\ldots,L\}\) to index completion positions. In our setting, the tokenizer, multimodal encoder, and backbone parameterization are inherited from the source VLM; the main changes lie in the training target and decoding pattern.

\subsection{From Autoregressive VLMs to dVLMs}
A standard autoregressive VLM is trained with next-token prediction:
\begin{equation}
\mathcal{L}_{\mathrm{AR}}(\phi)
=
-
\mathbb{E}_{(Q,x_1)\sim p_{\rm data}}
\left[
\sum_{i=1}^{L}
\log p_\phi(x_{1,i}\mid x_{1,<i}, Q)
\right],
\label{eq:ar_loss}
\end{equation}
where \(\phi\) denotes the parameters of the source VLM. In this formulation, the model predicts the next token under a causal prefix state.

A dVLM instead predicts clean tokens from a corrupted completion state \(x_t\). The bridge from VLM to dVLM therefore replaces next-token prediction with same-position denoising:
\begin{equation}
p_\theta(x_{1,i}\mid x_t, Q), \qquad i\in\mathcal{C},
\label{eq:dvml_denoise}
\end{equation}
where \(\theta\) denotes the parameters of the diffusion model. This change is substantial even when the model architecture is kept identical, because the student no longer operates on causal prefix states and will later be decoded with blockwise parallel refinement rather than token-by-token generation.

\subsection{Discrete Diffusion}
\faCheckSquareO \textcolor{green}{
1) Mask diffusion...
2) Uniform diffusion...
Highlight: we support both diffusion paradigms and proposed a mixture noise paradigm.}
Discrete diffusion models differ mainly in how they corrupt the clean completion \(x_1\) into an intermediate state \(x_t\). A convenient position-wise form is
\begin{equation}
q(x_t^i \mid x_1^i, t)
=
\alpha_t \, \delta_{\texttt{[MASK]}}(x_t^i)
+
\beta_t \, p_u(x_t^i)
+
(1-\alpha_t-\beta_t)\,\delta_{x_1^i}(x_t^i),
\qquad i\in\mathcal{C},
\label{eq:generic_corruption}
\end{equation}
where \(p_u\) is a uniform distribution over the vocabulary (excluding \texttt{[MASK]}), and \(\delta_a(\cdot)\) denotes a point mass at token \(a\).

This form recovers several common diffusion paradigms. Absorbing-state masked diffusion corresponds to \(\beta_t=0\), so corrupted positions are replaced by \texttt{[MASK]}. Uniform-token diffusion corresponds to \(\alpha_t=0\), so corrupted positions are replaced by random visible tokens. Later in the paper, we also study a mixed-noise variant with both \(\alpha_t>0\) and \(\beta_t>0\) as an optional refinement, but it is not required by the main bridging framework.

In the main bridge, we use the standard absorbing-state objective for stability. Specifically, \(x_t \sim q(x_t\mid x_1)\) is obtained by independently replacing each token in \(x_1\) with \texttt{[MASK]} with probability \(t\), where \(t \sim \mathrm{U}(0,1)\) \cite{sahoo2024simple,ou2024your}. Under this corruption process, maximizing the ELBO reduces to a reweighted cross-entropy over masked positions:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\mathrm{mask}}(\theta)
&=
\mathbb{E}_{(Q,x_1)\sim p_{\rm data},\, x_t \sim q(x_t \mid x_1),\, t \sim \mathrm{U}(0,1)} \\
& \left[
-\frac{1}{t}\sum_{\ell=1}^{L}
\mathbf{1}_{\{x_{t,\ell}=\text{\texttt{[MASK]}}\}}
\log p_\theta(x_{1,\ell}\mid x_t, Q)
\right].
\end{aligned}
\label{eq:mask_loss}
\end{equation}
Compared with Eq.~\eqref{eq:ar_loss}, the target is now position-aligned rather than next-token shifted, and the model is trained to reconstruct clean tokens from corrupted completion states.

\subsection{Blockwise Parallel Decoding}

At inference time, dVLMs commonly use blockwise decoding to support open-ended generation while exposing parallelism within each active block \cite{arriola2025block,li2025lavida,zeng2025diffusionvl}. Let \(\mathcal{B}_m \subseteq \mathcal{C}\) denote the current block, and let \(x^{(s)}\) be its partially denoised state at refinement step \(s\). Denote by \(\mathcal{M}^{(s)} \subseteq \mathcal{B}_m\) the masked positions in the current block. For each \(i \in \mathcal{M}^{(s)}\), the model predicts
\begin{equation}
\begin{aligned}
\hat{x}_i^{(s)} &= \arg\max_{v\in\mathcal V} p_\theta(x_i=v \mid x^{(s)}, Q), \\
c_i^{(s)} &= \max_{v\in\mathcal V} p_\theta(x_i=v \mid x^{(s)}, Q), \\
U^{(s)} &= \{ i\in\mathcal{M}^{(s)} : c_i^{(s)}\ge\eta\},
\end{aligned}
\label{eq:confidence_schedule}
\end{equation}
where \(\eta \in (0,1)\) is a confidence threshold that controls how many masked tokens are materialized at each step. Standard decoding finalizes tokens in \(U^{(s)}\) and leaves the remaining masked positions for later refinement.

The block size acts as a direct control knob for the bridge from autoregressive to diffusion decoding. When the block size is small, decoding remains closer to the autoregressive regime; when the block size is large, more tokens can be updated in parallel and diffusion decoding becomes substantially faster, but optimization also becomes more fragile. Unlike full-sequence diffusion, blockwise decoding additionally preserves arbitrary-length generation by appending new blocks on demand.

Taken together, Eqs.~\eqref{eq:ar_loss}, \eqref{eq:mask_loss}, and \eqref{eq:confidence_schedule} clarify the bridging problem studied in this paper. Converting an autoregressive VLM into a practical dVLM requires preserving model capability under two simultaneous changes: the training objective shifts from next-token prediction to same-position denoising, and the decoding process shifts from token-level causal rollout to blockwise parallel refinement. In the next section, we present a simple bridging framework based on progressive block scaling and stage-wise intra-dVLM distillation.
